A universal niche geometry governs the response of ecosystems to environmental perturbations

How ecosystems respond to environmental perturbations is a fundamental question in ecology, made especially challenging due to the strong coupling between species and their environment. Here, we introduce a theoretical framework for calculating the steady-state response of ecosystems to environmental perturbations in generalized consumer-resource. Our construction is applicable to a wide class of systems, including models with non-reciprocal interactions, cross-feeding, and non-linear growth/consumption rates. Within our framework, all ecological variables are embedded into four distinct vector spaces and ecological interactions are represented by geometric transformations between these spaces. We show that near a steady state, such geometric transformations directly map environmental perturbations - in resource availability and mortality rates - to shifts in niche structure. We illustrate these ideas in a variety of settings including a minimal model for pH-induced toxicity in bacterial denitrification. We end by discussing the biological implications of our framework. In particular, we show that it is extremely difficult to distinguish cooperative and competitive interactions by measuring species' responses to external perturbations.

==> reviewer_response/cover_letter.tex <==
Dear \editorname,

Please find enclosed the revised version of our previous submission entitled \enquote{\thetitle} with manuscript number \manuscript. We would like to thank you and the reviewers for the taking the time to carefully engage with our manuscript. We took these extensive comments to heart and  substantially re-hauled the manuscript. The revised version contains a major new section and figure in the main text, new analyses, a clearer methods section, as well as significant streamlining of the main text. We also provide new code (in the form of an attached Python notebook) and statistical results to clarify that our statement about the differential sensitivity of generalists and specialists holds. 

Specifically, the new section V explicitly contains biological insights  about ecosystems that our framework uniquely provides. These include showing that it is extremely difficult to distinguish a competitive community from a cooperative one by perturbing a community (Fig. 5). Other new insights include explaining why simple consumer-resource models are often successful in capturing  observed community phenomena even when we know that the underlying mechanistic processes are qualitatively more complex, and providing a rigorous mathematical definition of niches as a geometric quantity.

We believe that these changes significantly strengthen our manuscript and address virtually all the criticisms of the reviewers. We hope that our manuscript is now suitable for publication in \emph{PRX Life}.



\vspace{1.2em}

Sincerely,

\vspace{1.5em}

\theauthor

\vfil
\textbf{Note:} For clarity, each comment is displayed in a blue box, and additions/changes to the manuscript are in gray boxes.
